MMO: Meta Multi-Objectivization for Software Configuration Tuning

Software configuration tuning is essential for optimizing a given performance objective (e.g., minimizing latency). Yet, due to the software's intrinsically complex configuration landscape and expensive measurement, there has been a rather mild success, particularly in preventing the search from being trapped in local optima. To address this issue, in this paper we take a different perspective. Instead of focusing on improving the optimizer, we work on the level of optimization model and propose a meta multi-objectivization (MMO) model that considers an auxiliary performance objective (e.g., throughput in addition to latency). What makes this model distinct is that we do not optimize the auxiliary performance objective, but rather use it to make similarly-performing while different configurations less comparable (i.e. Pareto nondominated to each other), thus preventing the search from being trapped in local optima. Importantly, by designing a new normalization method, we show how to effectively use the MMO model without worrying about its weight -- the only yet highly sensitive parameter that can affect its effectiveness. Experiments on 22 cases from 11 real-world software systems/environments confirm that our MMO model with the new normalization performs better than its state-of-the-art single-objective counterparts on 82% cases while achieving up to 2.09x speedup. For 68% of the cases, the new normalization also enables the MMO model to outperform the instance when using it with the normalization from our prior FSE work under pre-tuned best weights, saving a great amount of resources which would be otherwise necessary to find a good weight. We also demonstrate that the MMO model with the new normalization can consolidate recent model-based tuning tools on 68% of the cases with up to 1.22x speedup in general.

==> figures/details/before_points.tex <==
\begin{figure}[t!]
	\centering
	\begin{subfigure}[h]{0.31\columnwidth}
		\includegraphics[width=\textwidth]{figures/new_pic/w=0.5_old.pdf}
		\subcaption{\footnotesize Original}
	\end{subfigure}
	~
	\begin{subfigure}[h]{0.31\columnwidth}
		\includegraphics[width=\textwidth]{figures/new_pic/w=1_old.pdf}
		\subcaption{\footnotesize Normalized}
	\end{subfigure}
	~
	\begin{subfigure}[h]{0.31\columnwidth}
		\includegraphics[width=\textwidth]{figures/new_pic/w=2_old.pdf}
		\subcaption{\footnotesize In the MMO space}
	\end{subfigure}

		\caption{The same population of Figure~\ref{fig:lrzip-old} under the MMO model with the new normalization method proposed in this work.}
	%\caption{The same evolutionary population of Figure~\ref{fig:lrzip-old} under the MMO model with the new normalization method.}
	\label{fig:lrzip-new}
\end{figure}

==> tables/rq1-bk.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing MMO with the other state-of-the-arts over 50 runs. SO$_{best}$ and MMO/FSE$_{best}$ denote the best single-objective model/optimizer and the MMO/FSE with the best weight, respectively. \quartexp{0}{20}{10}{20} shows the average and standard deviation on the target performance objective achieved (all objective values are normalized within $[0,1]$ and the closer to the left, the better). \bquartexp{0}{20}{10}{20} denote the best average among others. Column ``$\hat{A}_{12}$ ($p$ value)'' shows the $\hat{A}_{12}$ and $p$ value when comparing the corresponding counterpart with MOO. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote MMO wins while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} mean it loses; otherwise it is a tie. The statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ (or $\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
    \label{tb:rq1}
    \footnotesize
    \setlength{\tabcolsep}{1mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc}
        \begin{tabular}{lcc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
SO$_{best}$&  \quart{29.95}{70.05}{64.98}{100} &\cellcolor{steel!30}\textbf{.76 ($<$.001)}\\ 
MMO/FSE$_{best}$&  \bquart{0.00}{68.84}{34.42}{100} &\cellcolor{red!10}\textbf{.36 ($<$.001)}\\ 
PMO&  \quart{33.97}{63.50}{65.72}{100} &\cellcolor{steel!30}\textbf{.70 ($<$.001)}\\ 
MMO&  \quart{5.69}{71.59}{41.48}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{0.00}{69.63}{34.82}{100} &{.50 ($=$.011)}\\ 
&  \quart{10.50}{40.36}{30.68}{100} &\cellcolor{steel!30}\textbf{.56 ($<$.001)}\\ 
&  \quart{17.31}{82.69}{58.66}{100} &\cellcolor{steel!30}\textbf{.95 ($<$.001)}\\ 
&  \bquart{10.18}{38.01}{29.18}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{12.10}{40.49}{32.34}{100} &\cellcolor{steel!30}{.53 ($<$.001)}\\ 
&  \bquart{16.35}{14.99}{23.84}{100} &\cellcolor{red!10}\textbf{.42 ($<$.001)}\\ 
&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.67 ($<$.001)}\\ 
&  \quart{12.73}{34.55}{30.01}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \bquart{3.82}{0.00}{3.82}{100} &{.50 ($=$1.00)}\\ 
&  \quart{25.68}{74.32}{62.84}{100} &\cellcolor{steel!30}\textbf{.99 ($<$.001)}\\ 
&  \quart{0.00}{24.32}{12.16}{100} &\cellcolor{steel!30}\textbf{.66 ($<$.001)}\\ 
&  \bquart{3.82}{0.00}{3.82}{100} &-\\ 
        \end{tabular}  \\
            (a). \textsc{MariaDB-O1}&& (b). \textsc{MariaDB-O2} && (c). \textsc{Storm/WC-O1}&& (d). \textsc{Storm/WC-O2}


        \\
        \\
           \begin{tabular}{lcccl}
          \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
SO$_{best}$&  \quart{8.13}{63.64}{39.95}{100} &\cellcolor{steel!30}\textbf{.68 ($<$.001)}\\ 
MMO/FSE$_{best}$&  \bquart{8.80}{9.67}{13.64}{100} &\cellcolor{red!10}\textbf{.40 ($<$.001)}\\ 
PMO&  \quart{40.88}{59.12}{70.44}{100} &\cellcolor{steel!30}\textbf{.94 ($<$.001)}\\ 
MMO&  \quart{0.00}{48.26}{24.13}{100} &-\\      
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
&  \quart{5.48}{17.73}{14.35}{100} &\cellcolor{steel!30}\textbf{.67 ($<$.001)}\\ 
&  \bquart{4.03}{12.29}{10.17}{100} &\cellcolor{red!10}\textbf{.35 ($<$.001)}\\ 
&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.98 ($<$.001)}\\ 
&  \quart{4.39}{14.18}{11.48}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{1.22}{45.04}{23.74}{100} &\cellcolor{steel!30}{.52 ($<$.001)}\\ 
&  \bquart{0.00}{37.23}{18.62}{100} &\cellcolor{red!10}{.48 ($<$.001)}\\ 
&  \quart{41.30}{58.70}{70.65}{100} &\cellcolor{steel!30}\textbf{.91 ($<$.001)}\\ 
&  \quart{0.68}{41.77}{21.57}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
&  \bquart{8.81}{0.00}{8.81}{100} &{.50 ($=$1.00)}\\ 
&  \quart{20.19}{79.81}{60.09}{100} &\cellcolor{steel!30}\textbf{.94 ($<$.001)}\\ 
&  \quart{0.00}{22.92}{11.46}{100} &\cellcolor{steel!30}{.53 ($<$.001)}\\ 
&  \bquart{8.81}{0.00}{8.81}{100} &-\\  
   
        \end{tabular}  \\ 
                (e). \textsc{VP9-O1}&& (f). \textsc{VP9-O2} && (g). \textsc{Storm/RS-O1}&& (h). \textsc{Storm/RS-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
SO$_{best}$&  \quart{17.02}{24.30}{29.17}{100} &\cellcolor{steel!30}\textbf{.63 ($<$.001)}\\ 
MMO/FSE$_{best}$&  \quart{22.28}{23.10}{33.83}{100} &\cellcolor{steel!30}\textbf{.83 ($<$.001)}\\ 
PMO&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.94 ($<$.001)}\\ 
MMO&  \bquart{19.37}{13.42}{26.08}{100} &-\\       
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

&  \quart{0.25}{98.10}{49.31}{100} &\cellcolor{steel!30}\textbf{.62 ($<$.001)}\\ 
&  \quart{15.24}{40.16}{35.32}{100} &\cellcolor{steel!30}\textbf{.84 ($<$.001)}\\ 
&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.91 ($<$.001)}\\ 
&  \bquart{6.71}{61.46}{34.45}{100} &-\\  
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{15.35}{84.65}{57.67}{100} &\cellcolor{steel!30}\textbf{.98 ($<$.001)}\\ 
&  \quart{6.20}{55.26}{33.83}{100} &\cellcolor{steel!30}\textbf{.62 ($=$.006)}\\ 
&  \quart{0.00}{94.17}{47.08}{100} &\cellcolor{steel!30}\textbf{.92 ($<$.001)}\\ 
&  \bquart{8.31}{43.02}{29.82}{100} &-\\     
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

&  \quart{10.57}{72.79}{46.96}{100} &\cellcolor{steel!30}\textbf{.80 ($<$.001)}\\ 
&  \quart{13.13}{71.92}{49.09}{100} &\cellcolor{steel!30}\textbf{.76 ($<$.001)}\\ 
&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.79 ($<$.001)}\\ 
&  \bquart{11.14}{65.26}{43.77}{100} &-\\  
        \end{tabular}  \\
            (i). \textsc{LRZIP-O1}&& (j). \textsc{LRZIP-O2} && (k). \textsc{MongoDB-O1}&& (l). \textsc{MongoDB-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
          SO$_{best}$&  \quart{11.61}{88.39}{55.81}{100} &\cellcolor{steel!30}\textbf{.83 ($<$.001)}\\ 
MMO/FSE$_{best}$&  \quart{0.00}{83.32}{41.66}{100} &\cellcolor{steel!30}{.51 ($<$.001)}\\ 
PMO&  \bquart{21.63}{18.77}{31.01}{100} &\cellcolor{red!10}{.41 ($=$.284)}\\ 
MMO&  \quart{0.03}{80.56}{40.31}{100} &-\\         
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
       &  \quart{0.78}{27.67}{14.61}{100} &\cellcolor{steel!30}\textbf{.61 ($<$.001)}\\ 
&  \quart{34.94}{65.06}{67.47}{100} &\cellcolor{steel!30}\textbf{.97 ($<$.001)}\\ 
&  \quart{5.38}{24.36}{17.56}{100} &\cellcolor{steel!30}\textbf{.72 ($<$.001)}\\ 
&  \bquart{0.00}{23.31}{11.66}{100} &-\\    
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{22.19}{77.81}{61.10}{100} &\cellcolor{steel!30}\textbf{.79 ($<$.001)}\\ 
&  \quart{7.48}{82.00}{48.48}{100} &\cellcolor{steel!30}\textbf{.64 ($<$.001)}\\ 
&  \bquart{16.80}{22.92}{28.26}{100} &\cellcolor{steel!30}{.55 ($=$.401)}\\ 
&  \quart{0.00}{80.06}{40.03}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
 &  \quart{19.22}{4.30}{21.37}{100} &\cellcolor{steel!30}\textbf{.65 ($<$.001)}\\ 
&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.99 ($<$.001)}\\ 
&  \quart{20.69}{4.29}{22.84}{100} &\cellcolor{steel!30}\textbf{.82 ($<$.001)}\\ 
&  \bquart{19.64}{1.06}{20.17}{100} &-\\     
        \end{tabular}  \\
             (n). \textsc{Keras-DNN/SA-O1}&& (m). \textsc{Keras-DNN/SA-O2} && (o). \textsc{Keras-DNN/Adiac-O1}&& (p). \textsc{Keras-DNN/Adiac-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
     SO$_{best}$&  \quart{22.89}{73.85}{59.82}{100} &\cellcolor{steel!30}\textbf{.88 ($<$.001)}\\ 
MMO/FSE$_{best}$&  \bquart{0.00}{100.00}{50.00}{100} &\cellcolor{red!10}\textbf{.20 ($<$.001)}\\ 
PMO&  \quart{59.30}{9.45}{64.02}{100} &\cellcolor{steel!30}\textbf{.90 ($<$.001)}\\ 
MMO&  \quart{21.53}{70.59}{56.83}{100} &-\\          
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
      &  \quart{10.46}{89.54}{55.23}{100} &\cellcolor{red!10}{.49 ($=$.010)}\\ 
&  \bquart{0.00}{75.90}{37.95}{100} &\cellcolor{red!10}\textbf{.23 ($<$.001)}\\ 
&  \quart{36.69}{47.88}{60.64}{100} &\cellcolor{steel!30}\textbf{.68 ($<$.001)}\\ 
&  \quart{15.39}{74.22}{52.50}{100} &-\\    
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
         &  \bquart{42.60}{0.00}{42.60}{100} &{.50 ($=$1.00)}\\ 
&  \bquart{42.60}{0.00}{42.60}{100} &{.50 ($=$1.00)}\\ 
&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}{.52 ($<$.001)}\\ 
&  \bquart{42.60}{0.00}{42.60}{100} &-\\    
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{3.59}{82.00}{44.59}{100} &\cellcolor{steel!30}\textbf{.79 ($<$.001)}\\ 
&  \quart{0.86}{74.03}{37.87}{100} &\cellcolor{steel!30}{.54 ($=$.385)}\\ 
&  \quart{39.93}{60.07}{69.97}{100} &\cellcolor{steel!30}\textbf{.96 ($<$.001)}\\ 
&  \bquart{0.00}{74.89}{37.45}{100} &-\\    
        \end{tabular}  \\
             (q). \textsc{x264-O1}&& (r). \textsc{x264-O2} && (s). \textsc{LLVM-O1}&& (t). \textsc{LLVM-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
     
SO$_{best}$&  \bquart{100}{0}{100}{100} &{.50 ($=$1.00)}\\ 
MMO/FSE$_{best}$& \bquart{100}{0}{100}{100} &{.50 ($=$1.00)}\\ 
PMO&   \bquart{100}{0}{100}{100} &{.50 ($=$1.00)}\\ 
MMO&   \bquart{100}{0}{100}{100} &-\\          
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{6.32}{58.35}{35.50}{100} &\cellcolor{steel!30}\textbf{.92 ($<$.001)}\\ 
&  \bquart{6.98}{39.31}{26.63}{100} &\cellcolor{red!10}\textbf{.40 ($=$.006)}\\ 
&  \quart{19.27}{80.73}{59.64}{100} &\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\ 
&  \quart{0.00}{58.57}{29.28}{100} &-\\ 
        \end{tabular} &
        
             \begin{minipage}{0.001\textwidth}
         \begin{tabular}{p{5.05cm}ccc}
              &   \textbf{\% Win}& \textbf{\% Lose} & \textbf{\% Tie}   \\
            \hline
MMO vs. SO$_{best}$&73\%&4\%&23\%\\ 
MMO vs. MMO/FSE$_{best}$&55\%&36\%&9\%\\ 
MMO vs. PMO&90\%&5\%&5\%\\ 
&&&\\ 
        \end{tabular}    
     \end{minipage}
        
        &
  
        &
   
         &
         
                
       \\
            (u). \textsc{Trimesh-O1}&& (v). \textsc{Trimesh-O2}  & \begin{minipage}{0.001\textwidth}
                        \begin{tabular}{c}
           (w). Overall \% win/loss/tie for MMO versus the others
        \end{tabular} 
                 \end{minipage}&
                 &&
        \\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/rq1-pairwise.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing MMO with the other state-of-the-arts over 50 runs. SO$_{best}$ and MMO-FSE$_{best}$ denote the best single-objective model/optimizer and the MMO-FSE with the best weight, respectively. \quartexp{0}{20}{10}{20} shows the average and standard error (SE) on the target performance objective achieved (all objective values are normalized within $[0,1]$ and the closer to the left, the better). \bquartexp{0}{20}{10}{20} denotes the best average among others. Column ``$\hat{A}_{12}$ ($p$ value)'' shows the $\hat{A}_{12}$ and $p$ value when comparing the corresponding counterpart with MMO. ``T'', ``S'', ``M'', and ``L'' denotes trivial, small, medium, and large effect size, respectively. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote MMO wins ($\hat{A}_{12} > 0.5$) while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} mean it loses ($\hat{A}_{12} < 0.5$); otherwise it is a tie ($\hat{A}_{12} = 0.5$). Statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ ($\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
    \label{tb:rq1}
    \footnotesize
    %\setlength{\tabcolsep}{1mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc}
        \begin{tabular}{lcc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

SO$_{best}$&  \quart{74.95}{24.36}{87.13}{100} &\cellcolor{steel!30}\textbf{.66 M ($=$.005)}\\ 
MMO-FSE$_{best}$&  \bquart{0.00}{23.94}{11.97}{100} &\cellcolor{red!10}{.43 M ($=$.197)}\\ 
PMO& \quart{77.91}{22.09}{88.96}{100} &\cellcolor{steel!30}\textbf{.65 M ($=$.011)}\\ 
MMO&  \quart{16.89}{24.90}{29.34}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{10.18}{25.55}{22.96}{100} &\cellcolor{steel!30}{.51 T ($=$.899)}\\ 
&  \quart{4.82}{14.81}{12.23}{100} &\cellcolor{steel!30}{.53 T ($=$.608)}\\ 
&  \quart{69.66}{30.34}{84.83}{100} &\cellcolor{steel!30}\textbf{.71 L ($<$.001)}\\ 
&  \bquart{0.00}{13.92}{6.96}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{19.53}{16.70}{27.88}{100} &\cellcolor{steel!30}{.55 T ($=$.366)}\\ 
&  \bquart{0.00}{6.18}{3.09}{100} &\cellcolor{red!10}{.46 T ($=$.491)}\\ 
&  \quart{58.75}{41.25}{79.38}{100} &\cellcolor{steel!30}\textbf{.66 M ($=$.005)}\\ 
&  \quart{6.89}{10.25}{12.01}{100} &-\\ 

        \end{tabular} &
        &
       \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \bquart{0.00}{0.00}{0.00}{100} &{.50 T ($=$1.00)}\\ 
&  \quart{83.65}{16.35}{91.82}{100} &\cellcolor{steel!30}\textbf{.99 L ($<$.001)}\\ 
&  \quart{10.30}{5.35}{12.97}{100} &\cellcolor{steel!30}\textbf{.66 M ($=$.006)}\\ 
&  \bquart{0.00}{0.00}{0.00}{100} &-\\  
        \end{tabular}  \\
            (a). \textsc{MariaDB-O1}&& (b). \textsc{MariaDB-O2} && (c). \textsc{Storm/WC-O1}&& (d). \textsc{Storm/WC-O2}


        \\
        \\
           \begin{tabular}{lcccl}
          \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
SO$_{best}$&   \quart{36.48}{14.60}{43.77}{100} &\cellcolor{steel!30}\textbf{.64 M ($=$.016)}\\ 
MMO-FSE$_{best}$&  \bquart{0.00}{2.22}{1.11}{100} &\cellcolor{red!10}{.44 S ($=$.279)}\\ 
PMO&   \quart{86.44}{13.56}{93.22}{100} &\cellcolor{steel!30}\textbf{.89 L ($<$.001)}\\ 
MMO& \quart{10.05}{10.57}{15.33}{100} &-\\

        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
&  \quart{7.40}{4.64}{9.72}{100} &\cellcolor{steel!30}\textbf{.64 M ($=$.018)}\\ 
&  \bquart{0.00}{3.64}{1.82}{100} &\cellcolor{red!10}{.48 T ($=$.754)}\\ 
&  \quart{70.39}{29.61}{85.20}{100} &\cellcolor{steel!30}\textbf{.87 L ($<$.001)}\\ 
&  \quart{1.79}{4.55}{4.06}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{10.72}{10.48}{15.96}{100} &\cellcolor{steel!30}{.57 M ($=$.228)}\\ 
&  \quart{3.19}{8.67}{7.52}{100} &\cellcolor{steel!30}{.52 T ($=$.720)}\\ 
&  \quart{86.34}{13.66}{93.17}{100} &\cellcolor{steel!30}\textbf{.90 L ($<$.001)}\\ 
&  \bquart{0.00}{6.87}{3.43}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
&  \bquart{0.00}{0.00}{0.00}{100} &{.50 T ($=$1.00)}\\ 
&  \quart{80.17}{19.83}{90.09}{100} &\cellcolor{steel!30}\textbf{.94 L ($<$.001)}\\ 
&  \quart{1.81}{5.69}{4.66}{100} &\cellcolor{steel!30}{.53 T ($=$.605)}\\ 
&  \bquart{0.00}{0.00}{0.00}{100} &-\\ 
   
        \end{tabular}  \\ 
                (e). \textsc{VP9-O1}&& (f). \textsc{VP9-O2} && (g). \textsc{Storm/RS-O1}&& (h). \textsc{Storm/RS-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

SO$_{best}$&  \quart{20.77}{13.56}{27.55}{100} &\cellcolor{steel!30}\textbf{.62 S ($=$.035)}\\
MMO-FSE$_{best}$&   \quart{23.95}{9.99}{28.95}{100} &\cellcolor{steel!30}\textbf{.77 L ($<$.001)}\\ 
PMO&  \quart{56.76}{43.24}{78.38}{100} &\cellcolor{steel!30}\textbf{.89 L ($<$.001)}\\ 
MMO&  \bquart{0.00}{6.51}{3.25}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

&  \quart{40.21}{56.42}{68.42}{100} &\cellcolor{steel!30}{.55 T ($=$.365)}\\ 
&  \quart{0.00}{43.10}{21.55}{100} &\cellcolor{steel!30}\textbf{.77 L ($<$.001)}\\ 
&  \quart{42.49}{57.51}{71.24}{100} &\cellcolor{steel!30}\textbf{.81 L ($<$.001)}\\ 
&  \bquart{2.51}{35.35}{20.19}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{65.79}{34.21}{82.90}{100} &\cellcolor{steel!30}\textbf{.74 L ($<$.001)}\\ 
&  \bquart{3.60}{22.33}{14.76}{100} &\cellcolor{steel!30}{.54 T ($=$.535)}\\ 
&  \quart{33.61}{38.05}{52.64}{100} &\cellcolor{steel!30}{.59 S ($=$.122)}\\ 
&  \quart{0.00}{39.96}{19.98}{100} &-\\    
        \end{tabular} &
        &   
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

&  \quart{50.40}{33.46}{67.13}{100} &\cellcolor{steel!30}\textbf{.63 S ($=$.031)}\\ 
&  \quart{57.53}{33.06}{74.06}{100} &\cellcolor{steel!30}\textbf{.64 M ($=$.018)}\\ 
&  \quart{54.03}{45.97}{77.01}{100} &\cellcolor{steel!30}{.60 S ($=$.076)}\\ 
&  \bquart{0.00}{37.83}{18.92}{100} &-\\  
        \end{tabular}  \\
            (i). \textsc{LRZIP-O1}&& (j). \textsc{LRZIP-O2} && (k). \textsc{MongoDB-O1}&& (l). \textsc{MongoDB-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
  
SO$_{best}$&  \quart{62.77}{37.23}{81.39}{100} &\cellcolor{steel!30}\textbf{.63 S ($=$.023)}\\ 
MMO-FSE$_{best}$&  \quart{21.71}{35.09}{39.25}{100} &\cellcolor{steel!30}{.54 T ($=$.493)}\\ 
PMO&   \bquart{3.59}{7.91}{7.54}{100} &\cellcolor{red!10}{.48 T ($=$.684)}\\ 
MMO&  \quart{0.00}{31.37}{15.69}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{9.98}{6.90}{13.43}{100} &\cellcolor{steel!30}\textbf{.62 S ($=$.037)}\\ 
&  \quart{84.87}{15.13}{92.43}{100} &\cellcolor{steel!30}\textbf{.94 L ($<$.001)}\\ 
&  \quart{7.51}{5.67}{10.34}{100} &\cellcolor{steel!30}\textbf{.61 S ($=$.049)}\\ 
&  \bquart{0.00}{6.24}{3.12}{100} &-\\   
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{72.46}{27.54}{86.23}{100} &\cellcolor{steel!30}\textbf{.65 M ($=$.012)}\\ 
&  \quart{40.15}{29.02}{54.66}{100} &\cellcolor{steel!30}{.54 T ($=$.517)}\\ 
&  \bquart{0.00}{8.11}{4.06}{100} &\cellcolor{steel!30}{.55 T ($=$.395)}\\ 
&  \quart{19.35}{28.34}{33.52}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{2.64}{1.64}{3.46}{100} &\cellcolor{steel!30}\textbf{.64 M ($=$.015)}\\ 
&  \quart{61.75}{38.25}{80.88}{100} &\cellcolor{steel!30}\textbf{.99 L ($<$.001)}\\ 
&  \quart{6.60}{1.64}{7.42}{100} &\cellcolor{steel!30}\textbf{.81 L ($<$.001)}\\ 
&  \bquart{0.00}{0.40}{0.20}{100} &-\\ 

        \end{tabular}  \\
             (n). \textsc{Keras-DNN/SA-O1}&& (m). \textsc{Keras-DNN/SA-O2} && (o). \textsc{Keras-DNN/Adiac-O1}&& (p). \textsc{Keras-DNN/Adiac-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
  
SO$_{best}$&   \quart{52.76}{47.24}{76.38}{100} &\cellcolor{steel!30}\textbf{.69 M ($=$.001)}\\ 
MMO-FSE$_{best}$&   \bquart{0.00}{63.97}{31.98}{100} &\cellcolor{red!10}{.45 T ($=$.370)}\\ 
PMO& \quart{92.38}{6.04}{95.40}{100} &\cellcolor{steel!30}\textbf{.67 M ($=$.004)}\\ 
MMO& \quart{40.29}{45.15}{62.86}{100} &-\\
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{51.90}{40.27}{72.04}{100} &\cellcolor{steel!30}\textbf{.61 S ($=$.049)}\\ 
&  \bquart{0.00}{34.14}{17.07}{100} &\cellcolor{steel!30}{.52 T ($=$.762)}\\ 
&  \quart{78.46}{21.54}{89.23}{100} &\cellcolor{steel!30}\textbf{.72 L ($<$.001)}\\ 
&  \quart{27.98}{53.61}{54.79}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \bquart{0.00}{0.00}{0.00}{100} &{.50 T ($=$1.00)}\\ 
&  \bquart{0.00}{0.00}{0.00}{100} &{.50 T ($=$1.00)}\\ 
&  \quart{2.28}{97.72}{51.14}{100} &\cellcolor{steel!30}{.52 T ($=$.730)}\\ 
&  \bquart{0.00}{0.00}{0.00}{100} &-\\  
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{30.17}{22.86}{41.60}{100} &\cellcolor{steel!30}\textbf{.62 S ($=$.043)}\\ 
&  \quart{18.04}{20.64}{28.36}{100} &\cellcolor{steel!30}{.59 S ($=$.107)}\\ 
&  \quart{83.25}{16.75}{91.63}{100} &\cellcolor{steel!30}\textbf{.78 L ($<$.001)}\\ 
&  \bquart{0.00}{18.72}{9.36}{100} &-\\   
        \end{tabular}  \\
             (q). \textsc{x264-O1}&& (r). \textsc{x264-O2} && (s). \textsc{LLVM-O1}&& (t). \textsc{LLVM-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
     
SO$_{best}$&  \bquart{100}{0}{100}{100} &{.50 T ($=$1.00)}\\ 
MMO-FSE$_{best}$& \bquart{100}{0}{100}{100} &{.50 T ($=$1.00)}\\ 
PMO&   \bquart{100}{0}{100}{100} &{.50 T ($=$1.00)}\\ 
MMO&   \bquart{100}{0}{100}{100} &-\\          
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{28.02}{17.48}{36.76}{100} &\cellcolor{steel!30}\textbf{.66 M ($=$.005)}\\ 
&  \quart{12.09}{11.78}{17.98}{100} &\cellcolor{steel!30}{.52 T ($=$.672)}\\ 
&  \quart{75.81}{24.19}{87.91}{100} &\cellcolor{steel!30}\textbf{.81 L ($<$.001)}\\ 
&  \bquart{0.00}{16.30}{8.15}{100} &-\\ 
        \end{tabular} &
        
             \begin{minipage}{0.001\textwidth}
         \begin{tabular}{p{5.05cm}ccc}
              &   \textbf{\% Win}& \textbf{\% Lose} & \textbf{\% Tie}   \\
            \hline
MMO vs. SO$_{best}$&82\%&0\%&18\%\\ 
MMO vs. MMO-FSE$_{best}$&67\%&23\%&10\%\\ 
MMO vs. PMO&90\%&5\%&5\%\\ 
&&&\\ 
        \end{tabular}    
     \end{minipage}
        
        &
  
        &
   
         &
         
                
       \\
            (u). \textsc{Trimesh-O1}&& (v). \textsc{Trimesh-O2}  & \begin{minipage}{0.001\textwidth}
                        \begin{tabular}{c}
           (w). Overall \% win/loss/tie for MMO versus the others based on $\hat{A}_{12}$
        \end{tabular} 
                 \end{minipage}&
                 &&
        \\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/rq1.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing MMO with the other state-of-the-arts over 50 runs. SO$_{best}$ and MMO-FSE$_{best}$ denote the best single-objective model/optimizer and the MMO-FSE with the best weight, respectively. \quartexp{0}{20}{10}{20} shows the average and standard error (SE) on the target performance objective achieved (all objective values are normalized within $[0,1]$ and the closer to the left, the better). \bquartexp{0}{20}{10}{20} denotes the best average among others. Column ``$\hat{A}_{12}$ ($p$ value)'' shows the $\hat{A}_{12}$ and $p$ value when comparing the corresponding counterpart with MMO. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote MMO wins while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} mean it loses; otherwise it is a tie. Statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ ($\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
    \label{tb:rq1}
    \footnotesize
    %\setlength{\tabcolsep}{1mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc}
        \begin{tabular}{lcc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

SO$_{best}$&  \quart{74.95}{24.36}{87.13}{100} &\cellcolor{steel!30}\textbf{.76 ($<$.001)}\\ 
MMO-FSE$_{best}$&  \bquart{0.00}{23.94}{11.97}{100} &\cellcolor{red!10}\textbf{.36 ($<$.001)}\\ 
PMO&  \quart{77.91}{22.09}{88.96}{100} &\cellcolor{steel!30}\textbf{.70 ($<$.001)}\\ 
MMO&  \quart{16.89}{24.90}{29.34}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{8.94}{25.91}{21.90}{100} &{.50 ($=$.011)}\\ 
&  \quart{3.51}{15.02}{11.02}{100} &\cellcolor{steel!30}\textbf{.56 ($<$.001)}\\ 
&  \quart{69.24}{30.76}{84.62}{100} &\cellcolor{steel!30}\textbf{.95 ($<$.001)}\\ 
&  \bquart{0.00}{14.14}{7.07}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{19.53}{16.70}{27.88}{100} &\cellcolor{steel!30}{.53 ($<$.001)}\\ 
&  \bquart{0.00}{6.18}{3.09}{100} &\cellcolor{red!10}\textbf{.42 ($<$.001)}\\ 
&  \quart{58.75}{41.25}{79.38}{100} &\cellcolor{steel!30}\textbf{.67 ($<$.001)}\\ 
&  \quart{13.94}{14.25}{21.06}{100} &-\\ 

        \end{tabular} &
        &
       \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \bquart{0.00}{0.00}{0.00}{100} &{.50 ($<$.001)}\\ 
&  \quart{83.65}{16.35}{91.82}{100} &\cellcolor{steel!30}\textbf{.99 ($<$.001)}\\ 
&  \quart{10.30}{5.35}{12.97}{100} &\cellcolor{steel!30}\textbf{.66 ($<$.001)}\\ 
&  \bquart{0.00}{0.00}{0.00}{100} &-\\  
        \end{tabular}  \\
            (a). \textsc{MariaDB-O1}&& (b). \textsc{MariaDB-O2} && (c). \textsc{Storm/WC-O1}&& (d). \textsc{Storm/WC-O2}


        \\
        \\
           \begin{tabular}{lcccl}
          \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
SO$_{best}$&  \quart{36.48}{14.60}{43.77}{100} &\cellcolor{steel!30}\textbf{.68 ($<$.001)}\\ 
MMO-FSE$_{best}$&  \bquart{0.00}{2.22}{1.11}{100} &\cellcolor{red!10}\textbf{.40 ($<$.001)}\\ 
PMO&  \quart{86.44}{13.56}{93.22}{100} &\cellcolor{steel!30}\textbf{.94 ($<$.001)}\\ 
MMO&  \quart{12.59}{11.07}{18.12}{100} &-\\ 

        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
&  \quart{7.93}{5.25}{10.56}{100} &\cellcolor{steel!30}\textbf{.67 ($<$.001)}\\ 
&  \bquart{0.00}{3.64}{1.82}{100} &\cellcolor{red!10}\textbf{.35 ($<$.001)}\\ 
&  \quart{70.39}{29.61}{85.20}{100} &\cellcolor{steel!30}\textbf{.98 ($<$.001)}\\ 
&  \quart{2.45}{4.20}{4.55}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{7.78}{10.83}{13.19}{100} &\cellcolor{steel!30}{.52 ($<$.001)}\\ 
&  \bquart{0.00}{8.95}{4.48}{100} &\cellcolor{red!10}{.48 ($<$.001)}\\ 
&  \quart{85.89}{14.11}{92.94}{100} &\cellcolor{steel!30}\textbf{.91 ($<$.001)}\\ 
&  \quart{4.47}{10.04}{9.49}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
   
&  \bquart{0.00}{0.00}{0.00}{100} &{.50 ($<$.001)}\\ 
&  \quart{80.17}{19.83}{90.09}{100} &\cellcolor{steel!30}\textbf{.94 ($<$.001)}\\ 
&  \quart{1.81}{5.69}{4.66}{100} &\cellcolor{steel!30}{.53 ($<$.001)}\\ 
&  \bquart{0.00}{0.00}{0.00}{100} &-\\ 
   
        \end{tabular}  \\ 
                (e). \textsc{VP9-O1}&& (f). \textsc{VP9-O2} && (g). \textsc{Storm/RS-O1}&& (h). \textsc{Storm/RS-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

SO$_{best}$&  \quart{7.26}{10.76}{12.64}{100} &\cellcolor{steel!30}\textbf{.63 ($<$.001)}\\ 
MMO-FSE$_{best}$&  \quart{22.13}{10.23}{27.24}{100} &\cellcolor{steel!30}\textbf{.83 ($<$.001)}\\ 
PMO&  \quart{55.72}{44.28}{77.86}{100} &\cellcolor{steel!30}\textbf{.94 ($<$.001)}\\ 
MMO&  \bquart{0.00}{5.94}{2.97}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

&  \quart{40.21}{56.42}{68.42}{100} &\cellcolor{steel!30}\textbf{.62 ($<$.001)}\\ 
&  \quart{0.00}{63.10}{31.55}{100} &\cellcolor{steel!30}\textbf{.84 ($<$.001)}\\ 
&  \quart{42.49}{57.51}{71.24}{100} &\cellcolor{steel!30}\textbf{.91 ($<$.001)}\\ 
&  \bquart{2.51}{35.35}{20.19}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{67.53}{32.47}{83.77}{100} &\cellcolor{steel!30}\textbf{.98 ($<$.001)}\\ 
&  \quart{8.51}{21.19}{19.11}{100} &\cellcolor{steel!30}\textbf{.62 ($=$.006)}\\ 
&  \quart{37.00}{36.11}{55.05}{100} &\cellcolor{steel!30}\textbf{.92 ($<$.001)}\\ 
&  \bquart{0.00}{16.50}{8.25}{100} &-\\    
        \end{tabular} &
        &   
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

&  \quart{14.84}{57.46}{43.56}{100} &\cellcolor{steel!30}\textbf{.80 ($<$.001)}\\ 
&  \quart{27.08}{56.77}{55.47}{100} &\cellcolor{steel!30}\textbf{.76 ($<$.001)}\\ 
&  \quart{21.06}{78.94}{60.53}{100} &\cellcolor{steel!30}\textbf{.79 ($<$.001)}\\ 
&  \bquart{0.00}{51.52}{25.76}{100} &-\\  
        \end{tabular}  \\
            (i). \textsc{LRZIP-O1}&& (j). \textsc{LRZIP-O2} && (k). \textsc{MongoDB-O1}&& (l). \textsc{MongoDB-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
  
SO$_{best}$&  \quart{61.39}{38.61}{80.69}{100} &\cellcolor{steel!30}\textbf{.83 ($<$.001)}\\ 
MMO-FSE$_{best}$&  \quart{18.79}{36.40}{36.99}{100} &\cellcolor{steel!30}{.51 ($<$.001)}\\ 
PMO&  \bquart{0.00}{8.20}{4.10}{100} &\cellcolor{red!10}{.41 ($=$.284)}\\ 
MMO&  \quart{15.21}{35.19}{32.81}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{4.27}{6.31}{7.42}{100} &\cellcolor{steel!30}\textbf{.61 ($<$.001)}\\ 
&  \quart{85.18}{14.82}{92.59}{100} &\cellcolor{steel!30}\textbf{.97 ($<$.001)}\\ 
&  \quart{9.40}{5.55}{12.17}{100} &\cellcolor{steel!30}\textbf{.72 ($<$.001)}\\ 
&  \bquart{0.00}{5.31}{2.66}{100} &-\\    
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{72.46}{27.54}{86.23}{100} &\cellcolor{steel!30}\textbf{.79 ($<$.001)}\\ 
&  \quart{40.15}{29.02}{54.66}{100} &\cellcolor{steel!30}\textbf{.64 ($<$.001)}\\ 
&  \quart{0.00}{88.11}{44.06}{100} &\cellcolor{steel!30}{.55 ($=$.401)}\\ 
&  \bquart{19.35}{28.34}{33.52}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{2.64}{1.64}{3.46}{100} &\cellcolor{steel!30}\textbf{.65 ($<$.001)}\\ 
&  \quart{61.75}{38.25}{80.88}{100} &\cellcolor{steel!30}\textbf{.99 ($<$.001)}\\ 
&  \quart{6.60}{1.64}{7.42}{100} &\cellcolor{steel!30}\textbf{.82 ($<$.001)}\\ 
&  \bquart{0.00}{0.40}{0.20}{100} &-\\     
        \end{tabular}  \\
             (n). \textsc{Keras-DNN/SA-O1}&& (m). \textsc{Keras-DNN/SA-O2} && (o). \textsc{Keras-DNN/Adiac-O1}&& (p). \textsc{Keras-DNN/Adiac-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
  
SO$_{best}$&  \quart{52.76}{47.24}{76.38}{100} &\cellcolor{steel!30}\textbf{.88 ($<$.001)}\\ 
MMO-FSE$_{best}$&  \bquart{0.00}{63.97}{31.98}{100} &\cellcolor{red!10}\textbf{.20 ($<$.001)}\\ 
PMO&  \quart{92.38}{6.04}{95.40}{100} &\cellcolor{steel!30}\textbf{.90 ($<$.001)}\\ 
MMO&  \quart{40.29}{45.15}{62.86}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{51.90}{40.27}{72.04}{100} &\cellcolor{red!10}{.49 ($=$.010)}\\ 
&  \bquart{0.00}{34.14}{17.07}{100} &\cellcolor{red!10}\textbf{.23 ($<$.001)}\\ 
&  \quart{78.46}{21.54}{89.23}{100} &\cellcolor{steel!30}\textbf{.68 ($<$.001)}\\ 
&  \quart{46.65}{33.38}{63.34}{100} &-\\   
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
       &  \bquart{0.00}{0.00}{0.00}{100} &{.50 ($<$.001)}\\ 
&  \bquart{0.00}{0.00}{0.00}{100} &{.50 ($<$.001)}\\ 
&  \quart{2.28}{97.72}{51.14}{100} &\cellcolor{steel!30}{.52 ($<$.001)}\\ 
&  \bquart{0.00}{0.00}{0.00}{100} &-\\   
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{15.79}{27.57}{29.57}{100} &\cellcolor{steel!30}\textbf{.79 ($<$.001)}\\ 
&  \quart{1.16}{24.89}{13.60}{100} &\cellcolor{steel!30}{.54 ($=$.385)}\\ 
&  \quart{79.81}{20.19}{89.90}{100} &\cellcolor{steel!30}\textbf{.96 ($<$.001)}\\ 
&  \bquart{0.00}{25.18}{12.59}{100} &-\\    
        \end{tabular}  \\
             (q). \textsc{x264-O1}&& (r). \textsc{x264-O2} && (s). \textsc{LLVM-O1}&& (t). \textsc{LLVM-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
     
SO$_{best}$&  \bquart{100}{0}{100}{100} &{.50 ($=$1.00)}\\ 
MMO-FSE$_{best}$& \bquart{100}{0}{100}{100} &{.50 ($=$1.00)}\\ 
PMO&   \bquart{100}{0}{100}{100} &{.50 ($=$1.00)}\\ 
MMO&   \bquart{100}{0}{100}{100} &-\\          
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SE} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{18.11}{19.89}{28.06}{100} &\cellcolor{steel!30}\textbf{.92 ($<$.001)}\\ 
&  \bquart{0.00}{13.40}{6.70}{100} &\cellcolor{red!10}\textbf{.40 ($=$.006)}\\ 
&  \quart{72.48}{27.52}{86.24}{100} &\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\ 
&  \quart{3.10}{19.96}{13.09}{100} &-\\ 
        \end{tabular} &
        
             \begin{minipage}{0.001\textwidth}
         \begin{tabular}{p{5.05cm}ccc}
              &   \textbf{\% Win}& \textbf{\% Lose} & \textbf{\% Tie}   \\
            \hline
MMO vs. SO$_{best}$&73\%&4\%&23\%\\ 
MMO vs. MMO-FSE$_{best}$&55\%&36\%&9\%\\ 
MMO vs. PMO&90\%&5\%&5\%\\ 
&&&\\ 
        \end{tabular}    
     \end{minipage}
        
        &
  
        &
   
         &
         
                
       \\
            (u). \textsc{Trimesh-O1}&& (v). \textsc{Trimesh-O2}  & \begin{minipage}{0.001\textwidth}
                        \begin{tabular}{c}
           (w). Overall \% win/loss/tie for MMO versus the others based on $\hat{A}_{12}$
        \end{tabular} 
                 \end{minipage}&
                 &&
        \\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/rq3-copy.tex <==
\begin{table*}[t!]
\caption{Sensitivity analysis on different weights in the MMO model (full-scale experiments). The cells report the $\hat{A}_{12}$ values and whether $p<0.05$ on comparing a MMO instance and the best single-objective counterpart over 30 runs. The last row counts how many times a weight value is the best in a case based on Scott-Knott rank (primary) and the average result (secondary).}
\label{tb:sensitivity}
\setlength{\tabcolsep}{1.8mm}
\centering
\footnotesize
\begin{tabular}{lcccccccc||cccccccc}\toprule

\multirow{2}{*}{\textbf{Software System}}&\multicolumn{8}{c||}{\textbf{{MMO$+$ and MMO with NSGA-II}}}&\multicolumn{8}{c}{\textbf{{MMO$+$ and MMO with IBEA}}}\\ \cmidrule{2-17}

&\textbf{0.01}&\textbf{0.1}&\textbf{0.3}&\textbf{0.5}&\textbf{0.7}&\textbf{0.9}&\textbf{1.0}&\textbf{10}&\textbf{0.01}&\textbf{0.1}&\textbf{0.3}&\textbf{0.5}&\textbf{0.7}&\textbf{0.9}&\textbf{1.0}&\textbf{10}\\

\midrule

\textsc{MariaDB-O1}&\cellcolor{steel!30}\textbf{.60$^\dagger$}&\cellcolor{steel!30}\textbf{.56$^\dagger$}&\cellcolor{red!10}\textbf{.43$^\dagger$}&\cellcolor{steel!30}{.54$^\dagger$}&\cellcolor{red!10}{.49$^\dagger$}&\cellcolor{steel!30}\textbf{.58$^\dagger$}&\cellcolor{steel!30}{.52$^\dagger$}&\cellcolor{steel!30}\textbf{.96$^\dagger$}&\cellcolor{steel!30}{.51$^\dagger$}&\cellcolor{red!10}{.47$^\dagger$}&\cellcolor{red!10}{.45$^\dagger$}&\cellcolor{red!10}\textbf{.43$^\dagger$}&\cellcolor{red!10}{.49$^\dagger$}&\cellcolor{steel!30}{.54$^\dagger$}&\cellcolor{steel!30}{.54$^\dagger$}&\cellcolor{steel!30}{.54$^\dagger$}\\
\textsc{MariaDB-O2}&\cellcolor{red!10}{.50$^\dagger$}&\cellcolor{steel!30}\textbf{.56$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}\textbf{.61$^\dagger$}&\cellcolor{steel!30}\textbf{.60$^\dagger$}&\cellcolor{steel!30}\textbf{.65$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.72$^\dagger$}&\cellcolor{steel!30}{.52$^\dagger$}&\cellcolor{steel!30}\textbf{.57$^\dagger$}&\cellcolor{steel!30}\textbf{.60$^\dagger$}&\cellcolor{steel!30}\textbf{.63$^\dagger$}&\cellcolor{steel!30}\textbf{.61$^\dagger$}&\cellcolor{steel!30}\textbf{.65$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.71$^\dagger$}\\
\textsc{Storm/WC-O1}&\cellcolor{steel!30}\textbf{.56$^\dagger$}&\cellcolor{steel!30}{.54$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}\textbf{.60$^\dagger$}&\cellcolor{red!10}{.47$^\dagger$}&\cellcolor{red!10}{.45$^\dagger$}&\cellcolor{red!10}{.48$^\dagger$}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}{.54$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{red!10}\textbf{.40$^\dagger$}&\cellcolor{red!10}\textbf{.40$^\dagger$}&\cellcolor{steel!30}\textbf{.57$^\dagger$}\\
\textsc{Storm/WC-O2}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{.71$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}\\
\textsc{VP9-O1}&\cellcolor{steel!30}\textbf{.57$^\dagger$}&\cellcolor{red!10}\textbf{.44$^\dagger$}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{steel!30}\textbf{.62$^\dagger$}&\cellcolor{steel!30}\textbf{.74$^\dagger$}&\cellcolor{steel!30}\textbf{.85$^\dagger$}&\cellcolor{steel!30}\textbf{.87$^\dagger$}&\cellcolor{steel!30}\textbf{.93$^\dagger$}&\cellcolor{steel!30}{.51$^\dagger$}&\cellcolor{red!10}\textbf{.35$^\dagger$}&\cellcolor{red!10}{.48$^\dagger$}&\cellcolor{red!10}{.44$^\dagger$}&\cellcolor{red!10}{.49$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}\textbf{.56$^\dagger$}&\cellcolor{steel!30}\textbf{.82$^\dagger$}\\
\textsc{VP9-O2}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{red!10}{.49$^\dagger$}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}\textbf{.71$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.74$^\dagger$}&\cellcolor{steel!30}\textbf{.65$^\dagger$}&\cellcolor{steel!30}\textbf{.91$^\dagger$}&\cellcolor{red!10}{.50$^\dagger$}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{steel!30}\textbf{.62$^\dagger$}&\cellcolor{steel!30}\textbf{.58$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.67$^\dagger$}&\cellcolor{steel!30}\textbf{.76$^\dagger$}\\
\textsc{Storm/RS-O1}&\cellcolor{steel!30}{.54$^\dagger$}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{steel!30}\textbf{.57$^\dagger$}&\cellcolor{steel!30}{.56$^\dagger$}&\cellcolor{steel!30}{.56$^\dagger$}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}\textbf{.74$^\dagger$}&\cellcolor{steel!30}\textbf{.57$^\dagger$}&\cellcolor{red!10}{.49$^\dagger$}&\cellcolor{steel!30}{.54$^\dagger$}&{.50$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}\textbf{.69$^\dagger$}\\
\textsc{Storm/RS-O2}&\cellcolor{steel!30}\textbf{.94$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&{.50$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}\\
\textsc{LRZIP-O1}&\cellcolor{steel!30}\textbf{.73$^\dagger$}&\cellcolor{steel!30}\textbf{.97$^\dagger$}&\cellcolor{steel!30}\textbf{.98$^\dagger$}&\cellcolor{steel!30}\textbf{.98$^\dagger$}&\cellcolor{steel!30}\textbf{.98$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{.57$^\dagger$}&\cellcolor{steel!30}\textbf{.68$^\dagger$}&\cellcolor{steel!30}\textbf{.74$^\dagger$}&\cellcolor{steel!30}\textbf{.76$^\dagger$}&\cellcolor{steel!30}\textbf{.78$^\dagger$}&\cellcolor{steel!30}\textbf{.79$^\dagger$}&\cellcolor{steel!30}\textbf{.81$^\dagger$}&\cellcolor{steel!30}\textbf{.93$^\dagger$}\\
\textsc{LRZIP-O2}&\cellcolor{steel!30}{.51$^\dagger$}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{steel!30}\textbf{.77$^\dagger$}&\cellcolor{steel!30}\textbf{.84$^\dagger$}&\cellcolor{steel!30}\textbf{.84$^\dagger$}&\cellcolor{steel!30}\textbf{.84$^\dagger$}&\cellcolor{steel!30}\textbf{.85$^\dagger$}&\cellcolor{steel!30}\textbf{.90$^\dagger$}&\cellcolor{steel!30}{.50$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.70$^\dagger$}&\cellcolor{steel!30}\textbf{.75$^\dagger$}&\cellcolor{steel!30}\textbf{.79$^\dagger$}&\cellcolor{steel!30}\textbf{.83$^\dagger$}\\
\textsc{MongoDB-O1}&\cellcolor{steel!30}{.51}&\cellcolor{steel!30}\textbf{.61$^\dagger$}&\cellcolor{steel!30}{.60}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}{.57}&\cellcolor{steel!30}\textbf{.63$^\dagger$}&\cellcolor{steel!30}\textbf{.77$^\dagger$}&\cellcolor{steel!30}\textbf{.74$^\dagger$}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}\textbf{.63$^\dagger$}&\cellcolor{steel!30}\textbf{.61$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.62$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{.69$^\dagger$}\\
\textsc{MongoDB-O2}&\cellcolor{steel!30}{.57}&\cellcolor{steel!30}{.51}&\cellcolor{steel!30}{.59}&\cellcolor{steel!30}{.58}&\cellcolor{steel!30}{.60}&\cellcolor{steel!30}\textbf{.61$^\dagger$}&\cellcolor{steel!30}\textbf{.65$^\dagger$}&\cellcolor{steel!30}\textbf{.65$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}\textbf{.62$^\dagger$}&\cellcolor{steel!30}{.56$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{.70$^\dagger$}\\
\textsc{Keras-DNN/ShapesAll-O1}&\cellcolor{steel!30}{.55$^\dagger$}&\cellcolor{steel!30}{.51$^\dagger$}&\cellcolor{steel!30}{.50$^\dagger$}&\cellcolor{steel!30}\textbf{.67$^\dagger$}&\cellcolor{steel!30}\textbf{.67$^\dagger$}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}\textbf{.69$^\dagger$}&\cellcolor{steel!30}\textbf{.71$^\dagger$}&\cellcolor{steel!30}\textbf{.58$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}\textbf{.62$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}&\cellcolor{steel!30}\textbf{.78$^\dagger$}&\cellcolor{steel!30}\textbf{.72$^\dagger$}&\cellcolor{steel!30}\textbf{.77$^\dagger$}&\cellcolor{steel!30}\textbf{.74$^\dagger$}\\
\textsc{Keras-DNN/ShapesAll-O2}&\cellcolor{steel!30}\textbf{.95$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{.98$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{.97$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{.58$^\dagger$}&\cellcolor{steel!30}\textbf{.88$^\dagger$}&\cellcolor{steel!30}\textbf{.89$^\dagger$}&\cellcolor{steel!30}\textbf{.92$^\dagger$}&\cellcolor{steel!30}\textbf{.95$^\dagger$}&\cellcolor{steel!30}\textbf{.93$^\dagger$}&\cellcolor{steel!30}\textbf{.87$^\dagger$}&\cellcolor{steel!30}\textbf{.96$^\dagger$}\\
\textsc{Keras-DNN/Adiac-O1}&\cellcolor{steel!30}\textbf{.58$^\dagger$}&\cellcolor{red!10}{.47}&\cellcolor{steel!30}\textbf{.60$^\dagger$}&\cellcolor{steel!30}\textbf{.60$^\dagger$}&\cellcolor{steel!30}\textbf{.62$^\dagger$}&\cellcolor{steel!30}{.56$^\dagger$}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}\textbf{.65$^\dagger$}&\cellcolor{red!10}{.45}&\cellcolor{steel!30}{.51$^\dagger$}&\cellcolor{steel!30}\textbf{.62$^\dagger$}&\cellcolor{steel!30}\textbf{.61$^\dagger$}&\cellcolor{steel!30}\textbf{.70$^\dagger$}&\cellcolor{steel!30}\textbf{.71$^\dagger$}&\cellcolor{steel!30}\textbf{.65$^\dagger$}&\cellcolor{steel!30}\textbf{.66$^\dagger$}\\
\textsc{Keras-DNN/Adiac-O2}&\cellcolor{steel!30}\textbf{.98$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{.99$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}&\cellcolor{steel!30}\textbf{1.0$^\dagger$}\\
\textsc{x264-O1}&\cellcolor{red!10}{.48}&\cellcolor{red!10}{.44}&\cellcolor{red!10}{.48}&\cellcolor{steel!30}{.56$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{red!10}{.45}&\cellcolor{steel!30}{.54$^\dagger$}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{red!10}\textbf{.25$^\dagger$}&\cellcolor{red!10}\textbf{.21$^\dagger$}&\cellcolor{red!10}\textbf{.16$^\dagger$}&\cellcolor{red!10}\textbf{.17$^\dagger$}&\cellcolor{red!10}\textbf{.18$^\dagger$}&\cellcolor{red!10}\textbf{.19$^\dagger$}&\cellcolor{red!10}\textbf{.20$^\dagger$}&\cellcolor{red!10}\textbf{.22$^\dagger$}\\
\textsc{x264-O2}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{steel!30}{.51$^\dagger$}&\cellcolor{red!10}{.46}&\cellcolor{steel!30}{.51$^\dagger$}&\cellcolor{red!10}{.47$^\dagger$}&\cellcolor{steel!30}{.54$^\dagger$}&\cellcolor{steel!30}\textbf{.70$^\dagger$}&\cellcolor{steel!30}\textbf{.71$^\dagger$}&\cellcolor{steel!30}\textbf{.70$^\dagger$}&\cellcolor{steel!30}\textbf{.67$^\dagger$}&\cellcolor{steel!30}\textbf{.64$^\dagger$}&\cellcolor{steel!30}{.56$^\dagger$}&\cellcolor{steel!30}\textbf{.62$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}\\
\textsc{LLVM-O1}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&\cellcolor{steel!30}\textbf{.80$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&\cellcolor{steel!30}{.51$^\dagger$}\\
\textsc{LLVM-O2}&\cellcolor{steel!30}{.57}&\cellcolor{steel!30}{.54}&\cellcolor{steel!30}{.59}&\cellcolor{steel!30}{.59}&\cellcolor{steel!30}{.56}&\cellcolor{steel!30}{.55}&\cellcolor{steel!30}{.59}&\cellcolor{steel!30}{.58}&\cellcolor{steel!30}\textbf{.59$^\dagger$}&\cellcolor{steel!30}{.55}&\cellcolor{steel!30}{.56}&\cellcolor{steel!30}\textbf{.63$^\dagger$}&\cellcolor{steel!30}\textbf{.61$^\dagger$}&\cellcolor{steel!30}{.59}&\cellcolor{red!10}{.48}&\cellcolor{steel!30}\textbf{.66$^\dagger$}\\
\textsc{Trimesh-O1}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}&{.50$^\dagger$}\\
\textsc{Trimesh-O2}&\cellcolor{steel!30}{.52}&\cellcolor{red!10}{.46}&\cellcolor{steel!30}\textbf{.83$^\dagger$}&\cellcolor{steel!30}\textbf{.89$^\dagger$}&\cellcolor{steel!30}\textbf{.93$^\dagger$}&\cellcolor{steel!30}\textbf{.94$^\dagger$}&\cellcolor{steel!30}\textbf{.91$^\dagger$}&\cellcolor{steel!30}\textbf{.89$^\dagger$}&\cellcolor{steel!30}{.53$^\dagger$}&\cellcolor{red!10}{.38}&\cellcolor{steel!30}\textbf{.78$^\dagger$}&\cellcolor{steel!30}\textbf{.81$^\dagger$}&\cellcolor{steel!30}\textbf{.88$^\dagger$}&\cellcolor{steel!30}\textbf{.88$^\dagger$}&\cellcolor{steel!30}\textbf{.87$^\dagger$}&\cellcolor{steel!30}\textbf{.98$^\dagger$}\\




%\# Best&17&19&20&20&20&20&22&16&19&21&21&21&21&22&18&18&18&21&20&19&21\\

% sqaure get one 10 to 0.01
\bottomrule
\end{tabular}
%}
\centering
 \begin{tablenotes}
    \footnotesize
    \item $^\dagger$ denotes a statistically significant comparison with $p<0.05$. Other formats are the same as Table~\ref{tb:gain}.
    
    \end{tablenotes}
    \vspace{-0.3cm}
\end{table*}

==> tables/rq3-new.tex <==
\begin{table*}[t!]
\caption{$\hat{A}_{12}$ ($p$ value) on comparing MMO with MMO-FSE under different weights ($w$) over 50 runs. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote the cases where MMO wins while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} denote those that it loses; otherwise it is a tie. The statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ (or $\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
\label{tb:rq3}
%\setlength{\tabcolsep}{1.8mm}
\centering
\footnotesize
\begin{tabular}{lcccccccc}\toprule


\textbf{Software System}&$w=0.01$&$w=0.1$&$w=0.3$&$w=0.5$&$w=0.7$&$w=0.9$&$w=1$&$w=10$\\

\midrule

\textsc{MariaDB-O1}&\cellcolor{steel!30}{.60 ($=$.102)}&\cellcolor{steel!30}{.56 ($=$.287)}&\cellcolor{red!10}{.43 ($=$.197)}&\cellcolor{steel!30}{.54 ($=$.533)}&\cellcolor{red!10}{.49 ($=$.882)}&\cellcolor{steel!30}{.58 ($=$.178)}&\cellcolor{steel!30}{.52 ($=$.717)}&\cellcolor{steel!30}\textbf{.96 ($<$.001)}\\
\textsc{MariaDB-O2}&\cellcolor{steel!30}{.53 ($=$.608)}&\cellcolor{steel!30}{.60 ($=$.079)}&\cellcolor{steel!30}\textbf{.64 ($=$.019)}&\cellcolor{steel!30}\textbf{.66 ($=$.007)}&\cellcolor{steel!30}\textbf{.65 ($=$.010)}&\cellcolor{steel!30}\textbf{.69 ($<$.001)}&\cellcolor{steel!30}\textbf{.70 ($<$.001)}&\cellcolor{steel!30}\textbf{.75 ($<$.001)}\\
\textsc{Storm/WC-O1}&\cellcolor{steel!30}{.57 ($=$.212)}&\cellcolor{steel!30}{.55 ($=$.356)}&\cellcolor{steel!30}{.60 ($=$.071)}&\cellcolor{steel!30}{.61 ($=$.062)}&\cellcolor{red!10}{.48 ($=$.746)}&\cellcolor{red!10}{.46 ($=$.491)}&\cellcolor{red!10}{.49 ($=$.879)}&\cellcolor{steel!30}\textbf{.65 ($=$.012)}\\
\textsc{Storm/WC-O2}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{VP9-O1}&\cellcolor{steel!30}{.57 ($=$.197)}&\cellcolor{red!10}{.44 ($=$.279)}&\cellcolor{steel!30}{.55 ($=$.402)}&\cellcolor{steel!30}\textbf{.62 ($=$.043)}&\cellcolor{steel!30}\textbf{.74 ($<$.001)}&\cellcolor{steel!30}\textbf{.84 ($<$.001)}&\cellcolor{steel!30}\textbf{.86 ($<$.001)}&\cellcolor{steel!30}\textbf{.93 ($<$.001)}\\
\textsc{VP9-O2}&\cellcolor{steel!30}{.55 ($=$.396)}&\cellcolor{red!10}{.48 ($=$.754)}&\cellcolor{steel!30}\textbf{.64 ($=$.016)}&\cellcolor{steel!30}\textbf{.71 ($<$.001)}&\cellcolor{steel!30}\textbf{.65 ($=$.009)}&\cellcolor{steel!30}\textbf{.73 ($<$.001)}&\cellcolor{steel!30}\textbf{.65 ($=$.011)}&\cellcolor{steel!30}\textbf{.91 ($<$.001)}\\
\textsc{Storm/RS-O1}&\cellcolor{steel!30}{.53 ($=$.605)}&\cellcolor{steel!30}{.54 ($=$.491)}&\cellcolor{steel!30}{.56 ($=$.301)}&\cellcolor{steel!30}{.55 ($=$.389)}&\cellcolor{steel!30}{.55 ($=$.389)}&\cellcolor{steel!30}{.54 ($=$.491)}&\cellcolor{steel!30}{.52 ($=$.720)}&\cellcolor{steel!30}\textbf{.73 ($<$.001)}\\
\textsc{Storm/RS-O2}&\cellcolor{steel!30}\textbf{.94 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{LRZIP-O1}&\cellcolor{steel!30}\textbf{.77 ($<$.001)}&\cellcolor{steel!30}\textbf{.97 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}\\
\textsc{LRZIP-O2}&\cellcolor{steel!30}{.51 ($=$.820)}&\cellcolor{steel!30}{.55 ($=$.363)}&\cellcolor{steel!30}\textbf{.77 ($<$.001)}&\cellcolor{steel!30}\textbf{.84 ($<$.001)}&\cellcolor{steel!30}\textbf{.84 ($<$.001)}&\cellcolor{steel!30}\textbf{.84 ($<$.001)}&\cellcolor{steel!30}\textbf{.85 ($<$.001)}&\cellcolor{steel!30}\textbf{.90 ($<$.001)}\\
\textsc{MongoDB-O1}&\cellcolor{steel!30}{.54 ($=$.535)}&\cellcolor{steel!30}\textbf{.63 ($=$.022)}&\cellcolor{steel!30}\textbf{.62 ($=$.034)}&\cellcolor{steel!30}\textbf{.65 ($=$.010)}&\cellcolor{steel!30}\textbf{.65 ($=$.011)}&\cellcolor{steel!30}{.59 ($=$.105)}&\cellcolor{steel!30}\textbf{.65 ($=$.010)}&\cellcolor{steel!30}\textbf{.76 ($<$.001)}\\
\textsc{MongoDB-O2}&\cellcolor{steel!30}\textbf{.62 ($=$.034)}&\cellcolor{steel!30}{.58 ($=$.196)}&\cellcolor{steel!30}\textbf{.64 ($=$.016)}&\cellcolor{steel!30}\textbf{.63 ($=$.029)}&\cellcolor{steel!30}\textbf{.64 ($=$.018)}&\cellcolor{steel!30}\textbf{.65 ($=$.012)}&\cellcolor{steel!30}\textbf{.67 ($=$.003)}&\cellcolor{steel!30}\textbf{.67 ($=$.003)}\\
\textsc{Keras-DNN/SA-O1}&\cellcolor{steel!30}{.58 ($=$.166)}&\cellcolor{steel!30}{.55 ($=$.387)}&\cellcolor{steel!30}{.54 ($=$.493)}&\cellcolor{steel!30}\textbf{.73 ($<$.001)}&\cellcolor{steel!30}\textbf{.72 ($<$.001)}&\cellcolor{steel!30}\textbf{.69 ($=$.001)}&\cellcolor{steel!30}\textbf{.74 ($<$.001)}&\cellcolor{steel!30}\textbf{.75 ($<$.001)}\\
\textsc{Keras-DNN/SA-O2}&\cellcolor{steel!30}\textbf{.94 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{.96 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{Keras-DNN/Adiac-O1}&\cellcolor{steel!30}\textbf{.67 ($=$.004)}&\cellcolor{steel!30}{.54 ($=$.517)}&\cellcolor{steel!30}\textbf{.66 ($=$.004)}&\cellcolor{steel!30}\textbf{.64 ($=$.014)}&\cellcolor{steel!30}\textbf{.68 ($=$.002)}&\cellcolor{steel!30}\textbf{.62 ($=$.033)}&\cellcolor{steel!30}\textbf{.70 ($<$.001)}&\cellcolor{steel!30}\textbf{.71 ($<$.001)}\\
\textsc{Keras-DNN/Adiac-O2}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{x264-O1}&\cellcolor{red!10}{.48 ($=$.738)}&\cellcolor{red!10}{.44 ($=$.324)}&\cellcolor{red!10}{.48 ($=$.674)}&\cellcolor{steel!30}{.56 ($=$.334)}&\cellcolor{steel!30}{.59 ($=$.119)}&\cellcolor{red!10}{.45 ($=$.370)}&\cellcolor{steel!30}{.54 ($=$.540)}&\cellcolor{steel!30}{.59 ($=$.129)}\\
\textsc{x264-O2}&\cellcolor{steel!30}\textbf{.65 ($=$.009)}&\cellcolor{steel!30}{.59 ($=$.143)}&\cellcolor{steel!30}{.59 ($=$.120)}&\cellcolor{steel!30}{.57 ($=$.247)}&\cellcolor{steel!30}{.50 ($=$.956)}&\cellcolor{steel!30}{.57 ($=$.255)}&\cellcolor{steel!30}{.52 ($=$.762)}&\cellcolor{steel!30}{.58 ($=$.190)}\\
\textsc{LLVM-O1}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&\cellcolor{steel!30}\textbf{.80 ($<$.001)}\\
\textsc{LLVM-O2}&\cellcolor{steel!30}{.61 ($=$.062)}&\cellcolor{steel!30}{.59 ($=$.107)}&\cellcolor{steel!30}\textbf{.62 ($=$.036)}&\cellcolor{steel!30}\textbf{.63 ($=$.020)}&\cellcolor{steel!30}{.59 ($=$.127)}&\cellcolor{steel!30}{.59 ($=$.124)}&\cellcolor{steel!30}\textbf{.64 ($=$.019)}&\cellcolor{steel!30}{.59 ($=$.137)}\\
\textsc{Trimesh-O1}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}\\
\textsc{Trimesh-O2}&\cellcolor{steel!30}{.58 ($=$.186)}&\cellcolor{steel!30}{.52 ($=$.672)}&\cellcolor{steel!30}\textbf{.85 ($<$.001)}&\cellcolor{steel!30}\textbf{.90 ($<$.001)}&\cellcolor{steel!30}\textbf{.93 ($<$.001)}&\cellcolor{steel!30}\textbf{.94 ($<$.001)}&\cellcolor{steel!30}\textbf{.92 ($<$.001)}&\cellcolor{steel!30}\textbf{.91 ($<$.001)}\\


%\# Best&17&19&20&20&20&20&22&16&19&21&21&21&21&22&18&18&18&21&20&19&21\\

% sqaure get one 10 to 0.01
\bottomrule
\end{tabular}
%}
\centering

    \vspace{-0.3cm}
\end{table*}

==> tables/rq3.tex <==
\begin{table*}[t!]
\caption{$\hat{A}_{12}$ ($p$ value) on comparing MMO with MMO-FSE under different weights ($w$) over 50 runs. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote the cases where MMO wins while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} denote those that it loses; otherwise it is a tie. The statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ (or $\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
\label{tb:rq3}
%\setlength{\tabcolsep}{1.8mm}
\centering
\footnotesize
\begin{tabular}{lcccccccc}\toprule


\textbf{Software System}&$w=0.01$&$w=0.1$&$w=0.3$&$w=0.5$&$w=0.7$&$w=0.9$&$w=1$&$w=10$\\

\midrule

\textsc{MariaDB-O1}&\cellcolor{steel!30}\textbf{.67 ($<$.001)}&\cellcolor{steel!30}\textbf{.57 ($<$.001)}&\cellcolor{red!10}\textbf{.36 ($<$.001)}&\cellcolor{steel!30}{.54 ($<$.001)}&\cellcolor{red!10}{.46 ($<$.001)}&\cellcolor{steel!30}\textbf{.66 ($<$.001)}&\cellcolor{steel!30}{.55 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}\\
\textsc{MariaDB-O2}&\cellcolor{steel!30}\textbf{.56 ($<$.001)}&\cellcolor{steel!30}\textbf{.79 ($<$.001)}&\cellcolor{steel!30}\textbf{.84 ($<$.001)}&\cellcolor{steel!30}\textbf{.85 ($<$.001)}&\cellcolor{steel!30}\textbf{.83 ($<$.001)}&\cellcolor{steel!30}\textbf{.86 ($<$.001)}&\cellcolor{steel!30}\textbf{.86 ($<$.001)}&\cellcolor{steel!30}\textbf{.95 ($<$.001)}\\
\textsc{Storm/WC-O1}&\cellcolor{steel!30}{.55 ($<$.001)}&\cellcolor{steel!30}{.54 ($<$.001)}&\cellcolor{steel!30}\textbf{.60 ($<$.001)}&\cellcolor{steel!30}\textbf{.63 ($<$.001)}&\cellcolor{red!10}{.45 ($<$.001)}&\cellcolor{red!10}\textbf{.42 ($<$.001)}&\cellcolor{red!10}{.46 ($<$.001)}&\cellcolor{steel!30}\textbf{.69 ($<$.001)}\\
\textsc{Storm/WC-O2}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{VP9-O1}&{.50 ($=$.001)}&\cellcolor{red!10}\textbf{.40 ($<$.001)}&\cellcolor{steel!30}\textbf{.61 ($<$.001)}&\cellcolor{steel!30}\textbf{.68 ($<$.001)}&\cellcolor{steel!30}\textbf{.79 ($<$.001)}&\cellcolor{steel!30}\textbf{.87 ($<$.001)}&\cellcolor{steel!30}\textbf{.90 ($<$.001)}&\cellcolor{steel!30}\textbf{.94 ($<$.001)}\\
\textsc{VP9-O2}&\cellcolor{steel!30}{.55 ($<$.001)}&\cellcolor{red!10}\textbf{.35 ($<$.001)}&\cellcolor{steel!30}\textbf{.80 ($<$.001)}&\cellcolor{steel!30}\textbf{.90 ($<$.001)}&\cellcolor{steel!30}\textbf{.81 ($<$.001)}&\cellcolor{steel!30}\textbf{.95 ($<$.001)}&\cellcolor{steel!30}\textbf{.83 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}\\
\textsc{Storm/RS-O1}&\cellcolor{red!10}{.48 ($<$.001)}&\cellcolor{red!10}{.49 ($<$.001)}&\cellcolor{steel!30}{.51 ($<$.001)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&\cellcolor{red!10}{.49 ($<$.001)}&\cellcolor{red!10}{.48 ($<$.001)}&\cellcolor{steel!30}\textbf{.76 ($<$.001)}\\
\textsc{Storm/RS-O2}&\cellcolor{steel!30}\textbf{.94 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{LRZIP-O1}&\cellcolor{steel!30}\textbf{.83 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{LRZIP-O2}&\cellcolor{steel!30}\textbf{.56 ($<$.001)}&\cellcolor{steel!30}\textbf{.57 ($<$.001)}&\cellcolor{steel!30}\textbf{.84 ($<$.001)}&\cellcolor{steel!30}\textbf{.95 ($<$.001)}&\cellcolor{steel!30}\textbf{.93 ($<$.001)}&\cellcolor{steel!30}\textbf{.93 ($<$.001)}&\cellcolor{steel!30}\textbf{.96 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}\\
\textsc{MongoDB-O1}&\cellcolor{steel!30}\textbf{.62 ($=$.006)}&\cellcolor{steel!30}\textbf{.97 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{.94 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.90 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}\\
\textsc{MongoDB-O2}&\cellcolor{steel!30}\textbf{.80 ($<$.001)}&\cellcolor{steel!30}\textbf{.63 ($<$.001)}&\cellcolor{steel!30}\textbf{.93 ($<$.001)}&\cellcolor{steel!30}\textbf{.83 ($<$.001)}&\cellcolor{steel!30}\textbf{.76 ($<$.001)}&\cellcolor{steel!30}\textbf{.85 ($<$.001)}&\cellcolor{steel!30}\textbf{.87 ($<$.001)}&\cellcolor{steel!30}\textbf{.90 ($<$.001)}\\
\textsc{Keras-DNN/SA-O1}&\cellcolor{steel!30}\textbf{.72 ($<$.001)}&\cellcolor{steel!30}\textbf{.61 ($<$.001)}&\cellcolor{steel!30}{.51 ($<$.001)}&\cellcolor{steel!30}\textbf{.82 ($<$.001)}&\cellcolor{steel!30}\textbf{.73 ($<$.001)}&\cellcolor{steel!30}\textbf{.71 ($=$.006)}&\cellcolor{steel!30}\textbf{.84 ($<$.001)}&\cellcolor{steel!30}\textbf{.82 ($<$.001)}\\
\textsc{Keras-DNN/SA-O2}&\cellcolor{steel!30}\textbf{.97 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{Keras-DNN/Adiac-O1}&\cellcolor{steel!30}\textbf{.92 ($<$.001)}&\cellcolor{steel!30}\textbf{.64 ($<$.001)}&\cellcolor{steel!30}\textbf{.85 ($<$.001)}&\cellcolor{steel!30}\textbf{.83 ($<$.001)}&\cellcolor{steel!30}\textbf{.86 ($<$.001)}&\cellcolor{steel!30}\textbf{.79 ($<$.001)}&\cellcolor{steel!30}\textbf{.93 ($<$.001)}&\cellcolor{steel!30}\textbf{.80 ($<$.001)}\\
\textsc{Keras-DNN/Adiac-O2}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}\\
\textsc{x264-O1}&\cellcolor{red!10}\textbf{.36 ($<$.001)}&\cellcolor{red!10}\textbf{.23 ($<$.001)}&\cellcolor{red!10}\textbf{.38 ($<$.001)}&\cellcolor{steel!30}\textbf{.74 ($<$.001)}&\cellcolor{steel!30}\textbf{.85 ($<$.001)}&\cellcolor{red!10}\textbf{.20 ($<$.001)}&\cellcolor{steel!30}\textbf{.67 ($<$.001)}&\cellcolor{steel!30}\textbf{.81 ($<$.001)}\\
\textsc{x264-O2}&\cellcolor{steel!30}{.55 ($<$.001)}&\cellcolor{red!10}\textbf{.32 ($<$.001)}&\cellcolor{red!10}\textbf{.33 ($<$.001)}&\cellcolor{red!10}\textbf{.32 ($<$.001)}&\cellcolor{red!10}\textbf{.23 ($<$.001)}&\cellcolor{red!10}\textbf{.27 ($<$.001)}&\cellcolor{red!10}\textbf{.23 ($<$.001)}&\cellcolor{red!10}\textbf{.37 ($<$.001)}\\
\textsc{LLVM-O1}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&\cellcolor{steel!30}\textbf{.80 ($<$.001)}\\
\textsc{LLVM-O2}&\cellcolor{steel!30}\textbf{.72 ($=$.001)}&\cellcolor{steel!30}{.54 ($=$.385)}&\cellcolor{steel!30}\textbf{.83 ($<$.001)}&\cellcolor{steel!30}\textbf{.80 ($<$.001)}&\cellcolor{steel!30}\textbf{.65 ($=$.007)}&\cellcolor{steel!30}{.58 ($=$.101)}&\cellcolor{steel!30}\textbf{.71 ($<$.001)}&\cellcolor{steel!30}{.55 ($<$.001)}\\
\textsc{Trimesh-O1}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}&{.50 ($=$1.00)}\\
\textsc{Trimesh-O2}&\cellcolor{steel!30}\textbf{.61 ($<$.001)}&\cellcolor{red!10}\textbf{.40 ($=$.006)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}\\



%\# Best&17&19&20&20&20&20&22&16&19&21&21&21&21&22&18&18&18&21&20&19&21\\

% sqaure get one 10 to 0.01
\bottomrule
\end{tabular}
%}
\centering

    \vspace{-0.3cm}
\end{table*}

==> tables/rq4-bk.tex <==


% CS Table for RQ2
\begin{table*}[t!]
%\caption{Comparing \textsc{Flash} consolidated by our MOO$+$ model with the original \textsc{Flash} over 50 runs. The format is the same as Table~\ref{tb:rq1}.}
\caption{Comparing \textsc{Flash}-MMO and \textsc{Flash} over 50 runs. The format is the same as Table~\ref{tb:rq1}.}
    \label{tb:rq4}
    \footnotesize
    \setlength{\tabcolsep}{1mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc}
        \begin{tabular}{lcc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

\textsc{Flash}&  \quart{3.38}{96.62}{51.69}{100} &\cellcolor{steel!30}\textbf{.62 ($<$.001)}\\ 
\textsc{Flash-}MMO&  \bquart{0.00}{76.34}{38.17}{100} &-\\ 

        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \bquart{0.00}{97.54}{48.77}{100} &\cellcolor{red!10}{.48 ($=$.101)}\\ 
&  \quart{15.71}{84.29}{57.86}{100} &-\\ 

        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \bquart{0.00}{70.41}{35.20}{100} &\cellcolor{red!10}\textbf{.33 ($<$.001)}\\ 
&  \quart{3.91}{96.09}{51.95}{100} &-\\  
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{6.80}{93.20}{53.40}{100} &\cellcolor{steel!30}{.53 ($<$.001)}\\ 
&  \bquart{0.00}{99.41}{49.71}{100} &-\\ 
        \end{tabular}  \\
            (a). \textsc{MariaDB-O1}&& (b). \textsc{MariaDB-O2} && (c). \textsc{Storm/WC-O1}&& (d). \textsc{Storm/WC-O2}


        \\
        \\
           \begin{tabular}{lcccl}
          \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

\textsc{Flash}&  \bquart{11.04}{62.68}{42.38}{100} &\cellcolor{red!10}{.49 ($=$.530)}\\ 
\textsc{Flash-}MMO&  \quart{0.00}{100.00}{50.00}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{53.31}{46.69}{76.65}{100} &\cellcolor{steel!30}\textbf{.91 ($<$.001)}\\ 
&  \bquart{0.00}{64.63}{32.31}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
& \bquart{6.82}{52.71}{33.18}{100} &\cellcolor{red!10}\textbf{.31 ($<$.001)}\\ 
&  \quart{0.00}{100.00}{50.00}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.56 ($=$.040)}\\ 
&  \bquart{36.14}{13.83}{43.05}{100} &-\\ 
   
        \end{tabular}  \\ 
                (e). \textsc{VP9-O1}&& (f). \textsc{VP9-O2} && (g). \textsc{Storm/RS-O1}&& (h). \textsc{Storm/RS-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
\textsc{Flash}&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.58 ($=$.044)}\\ 
\textsc{Flash-}MMO&  \bquart{3.55}{93.02}{49.06}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{11.05}{88.95}{55.52}{100} &\cellcolor{steel!30}\textbf{.58 ($=$.015)}\\ 
&  \bquart{0.00}{92.79}{46.40}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{28.04}{71.96}{64.02}{100} &\cellcolor{steel!30}\textbf{.67 ($=$.008)}\\ 
&  \bquart{0.00}{92.56}{46.28}{100} &-\\  
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{15.39}{84.61}{57.69}{100} &\cellcolor{steel!30}\textbf{.73 ($<$.001)}\\ 
&  \bquart{0.00}{81.65}{40.83}{100} &-\\ 
        \end{tabular}  \\
            (i). \textsc{LRZIP-O1}&& (j). \textsc{LRZIP-O2} && (k). \textsc{MongoDB-O1}&& (l). \textsc{MongoDB-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
\textsc{Flash}&  \quart{20.69}{79.31}{60.34}{100} &\cellcolor{steel!30}\textbf{.63 ($=$.011)}\\ 
\textsc{Flash-}MMO&  \bquart{0.00}{85.41}{42.71}{100} &-\\ 
     
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}\textbf{.78 ($<$.001)}\\ 
&  \bquart{17.16}{9.04}{21.68}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{58.76}{23.01}{70.26}{100} &\cellcolor{steel!30}\textbf{.61 ($=$.005)}\\ 
&  \bquart{0.00}{100.00}{50.00}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{19.56}{62.67}{50.90}{100} &\cellcolor{steel!30}\textbf{.67 ($=$.002)}\\ 
&  \bquart{0.00}{100.00}{50.00}{100} &-\\
        \end{tabular}  \\
             (n). \textsc{Keras-DNN/SA-O1}&& (m). \textsc{Keras-DNN/SA-O2} && (o). \textsc{Keras-DNN/Adiac-O1}&& (p). \textsc{Keras-DNN/Adiac-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
               \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

\textsc{Flash}&  \bquart{0.00}{89.57}{44.79}{100} &\cellcolor{red!10}\textbf{.26 ($<$.001)}\\ 
\textsc{Flash-}MMO&  \quart{17.32}{82.68}{58.66}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \bquart{0.00}{87.85}{43.92}{100} &\cellcolor{red!10}\textbf{.36 ($<$.001)}\\ 
&  \quart{4.59}{95.41}{52.29}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \quart{9.38}{90.62}{54.69}{100} &\cellcolor{steel!30}\textbf{.78 ($<$.001)}\\ 
&  \bquart{0.00}{62.15}{31.08}{100} &-\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline
&  \bquart{0.34}{97.17}{48.93}{100} &\cellcolor{red!10}{.47 ($<$.001)}\\ 
&  \quart{0.00}{100.00}{50.00}{100} &-\\ 
        \end{tabular}  \\
             (q). \textsc{x264-O1}&& (r). \textsc{x264-O2} && (s). \textsc{LLVM-O1}&& (t). \textsc{LLVM-O2}
        \\
        
               \\
           \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

\textsc{Flash}&  \quart{0.00}{100.00}{50.00}{100} &\cellcolor{steel!30}{.51 ($<$.001)}\\ 
\textsc{Flash-}MMO&  \bquart{2.00}{87.97}{45.99}{100} &-\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{Mean/SD} & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)}  \\
            \hline

&  \quart{15.98}{80.70}{56.33}{100} &\cellcolor{steel!30}{.54 ($=$.103)}\\ 
&  \bquart{0.00}{100.00}{50.00}{100} &-\\ 
        \end{tabular} &
        
           \begin{minipage}{0.001\textwidth}
         \begin{tabular}{p{5.05cm}ccc}
              &   \textbf{\% Win}& \textbf{\% Lose} & \textbf{\% Tie}   \\
            \hline
\textsc{Flash-}MMO  vs. \textsc{Flash}&68\%&32\%&0\%\\ 
&&&\\ 
        \end{tabular}    
     \end{minipage}

        &
     
        &
       \\
            (u). \textsc{Trimesh-O1}&& (v). \textsc{Trimesh-O2}  & \begin{minipage}{0.001\textwidth}
                        \begin{tabular}{c}
           (w). Overall \% win/loss/tie for \textsc{Flash-}MMO versus \textsc{Flash}
        \end{tabular} 
                 \end{minipage}&&&
        \\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/sys.tex <==
\begin{table*}[t!]
%\caption{Configurable software systems studied.}
%\label{tb:sys}
%\setlength{\tabcolsep}{0.6mm}
\centering
\footnotesize

\begin{tabular}{cc}
\setlength{\tabcolsep}{1.2mm}
\begin{tabular}{lllll}


\multicolumn{5}{c}{\small TABLE 1: Configurable software systems studied.}\\

&&&&\\\toprule

\textbf{System}&\textbf{Domain}&\textbf{Performance Objective}&\textbf{$\lvert \mathbfcal{O} \rvert$}&\textbf{Search Space}\\

\midrule

\textsc{MariaDB}&SQL database&\textsc{O1:} latency; \textsc{O2:} CPU load&10&864\\

\cellcolor{steel!10}\textsc{Storm/WC}&\cellcolor{steel!10}stream processing&\cellcolor{steel!10}\textsc{O1:} throughput; \textsc{O2:} latency&\cellcolor{steel!10}6&\cellcolor{steel!10}2,880\\


\textsc{VP9}&video encoding&\textsc{O1:} latency; \textsc{O2:} CPU load&12&3,008\\


\cellcolor{steel!10}\textsc{Storm/RS}&\cellcolor{steel!10}stream processing&\cellcolor{steel!10}\textsc{O1:} throughput; \textsc{O2:} latency&\cellcolor{steel!10}6&\cellcolor{steel!10}3,839\\


\textsc{LRZIP}&file compression&\textsc{O1:} latency; \textsc{O2:} CPU load&12&5,184\\

\cellcolor{steel!10}\textsc{MongoDB}&\cellcolor{steel!10}no-SQL database&\cellcolor{steel!10}\textsc{O1:} latency; \textsc{O2:} CPU load&\cellcolor{steel!10}15&\cellcolor{steel!10}6,840\\

\textsc{Keras-DNN/SA}&deep learning&\textsc{O1:} AUC; \textsc{O2:} inference time&12&16,384\\

\cellcolor{steel!10}\textsc{Keras-DNN/Adiac}&\cellcolor{steel!10}deep learning&\cellcolor{steel!10}\textsc{O1:} AUC; \textsc{O2:} inference time&\cellcolor{steel!10}12&\cellcolor{steel!10}24,576\\


\textsc{x264}&video encoding&\textsc{O1:} PSNR; \textsc{O2:} energy usage&17&53,662\\


\cellcolor{steel!10}\textsc{LLVM}&\cellcolor{steel!10}compiler&\cellcolor{steel!10}\textsc{O1:} latency; \textsc{O2:} CPU load&\cellcolor{steel!10}16&\cellcolor{steel!10}65,436\\


\textsc{Trimesh}&triangle mesh&\textsc{O1:} \# iteration; \textsc{O2:} latency&13&239,260\\



%1.92$\times 10^{10}$

\bottomrule
\end{tabular}

&
\setlength{\tabcolsep}{1.2mm}
\begin{tabular}{lll}

\multicolumn{3}{c}{\small TABLE 2: Size and Budget.}\\

&&\\\toprule


\textbf{System}&\textbf{Size}&\textbf{Budget}\\\midrule
\textsc{MariaDB}&20&400\\
\cellcolor{steel!10}\textsc{Storm/WC}&\cellcolor{steel!10}50&\cellcolor{steel!10}600\\
\textsc{VP9}&30&700\\
\cellcolor{steel!10}\textsc{Storm/RS}&\cellcolor{steel!10}50&\cellcolor{steel!10}900\\
\textsc{LRZIP}&20&400\\
\cellcolor{steel!10}\textsc{MongoDB}&\cellcolor{steel!10}20&\cellcolor{steel!10}500\\
\textsc{Keras-DNN/SA}&20&400\\
\cellcolor{steel!10}\textsc{Keras-DNN/Adiac}&\cellcolor{steel!10}20&\cellcolor{steel!10}400\\
\textsc{x264}&50&2,500\\
\cellcolor{steel!10}\textsc{LLVM}&\cellcolor{steel!10}20&\cellcolor{steel!10}600\\
\textsc{Trimesh}&20&1,000\\

\bottomrule
\end{tabular}

\end{tabular}



%}
\centering
 \begin{tablenotes}
    \footnotesize
    %\item The configuration options are preprocessed and thus only the ones (and their ranges) that can affect the performance attributes are considered. 
    \item $\lvert \mathbfcal{O} \rvert$ denotes number of options. We run all systems under their standard benchmarks. More details can be found at: 
    %\href{https://github.com/taochen/mmo-fse-2021}{\texttt{\textcolor{blue}{https://github.com/taochen/mmo-fse-2021}}}.
    \end{tablenotes}
    % Notably, \textsc{Storm} and \textsc{Keras-DNN} have three benchmarks and two dataset, respectively.
\end{table*}

\setcounter{table}{2}
